Relaxed Gauss-Newton methods with applications to electrical impedance tomography

As second-order methods, Gauss--Newton-type methods can be more effective than first-order methods for the solution of nonsmooth optimization problems with expensive-to-evaluate smooth components. Such methods, however, often do not converge. Motivated by nonlinear inverse problems with nonsmooth regularization, we propose a new Gauss--Newton-type method with inexact relaxed steps. We prove that the method converges to a set of disjoint critical points given that the linearisation of the forward operator for the inverse problem is sufficiently precise. We extensively evaluate the performance of the method on electrical impedance tomography (EIT).

==> Figures/Layout/Case1.tex <==

\begin{figure}[!t]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim1/WT_Sim1_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim1/WT_Sim1_tvsJ".pdf}}%
    \caption{Case 1. \TextFigureJa}%
    \label{fig:WT_Sim1_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim1_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim1/WT_Sim1_w0.25".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim1/WT_Sim1_w0.75".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim1/WT_Sim1_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/WT_Sim1/WT_Sim1_Newton".pdf}%        
    \end{minipage}%
    \subfloatcolorbar{0.0cm}{-1.275cm}{2.55cm}{"Figures/WT_Sim1/WT_Sim1_Colorbar".pdf}%
    \caption{Case 1. \TextRecosa}%
    \label{fig:WT_Sim1_Recos}%
\end{figure}%


==> Figures/Layout/Case11.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_tvsJ".pdf}}%

    \caption{Case 11. \TextFigureJa}%

    \label{fig:Skin_Meas2_STV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas2_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_w0.5".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_w0.75".pdf}%     

        \subfloatreco{\ttAlgd}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_Newton".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/Skin_Meas2_STV/Skin_Meas2_STV_Colorbar".pdf}%
    \caption{Case 11. \TextRecosalld}%

    \label{fig:Skin_Meas2_STV_Recos}%
\end{figure}%


==> Figures/Layout/Case12.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJb]{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_tvsJ".pdf}}%

    \caption{Case 12. \TextFigureJc}%
    \label{fig:Skin_Meas2_TV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas2_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_w0.5".pdf}%
        
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_w0.75".pdf}% 
        \subfloatreco{\ttAlgd}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_w1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/Skin_Meas2_TV/Skin_Meas2_TV_Colorbar".pdf}%
    \caption{Case 12. \TextRecosalle}%
    \label{fig:Skin_Meas2_TV_Recos}%
\end{figure}%


==> Figures/Layout/Case1_all.tex <==

\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim1_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim1/WT_Sim1_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/WT_Sim1/WT_Sim1_w0.5".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim1/WT_Sim1_w0.75".pdf}%          
        
        \subfloatreco{\ttAlgd}{"Figures/WT_Sim1/WT_Sim1_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim1/WT_Sim1_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/WT_Sim1/WT_Sim1_Newton".pdf}%        
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/WT_Sim1/WT_Sim1_Colorbar".pdf}%
    \caption{Case 1. \TextRecosalla}%
    \label{fig:WT_Sim1_Recosall}%
\end{figure}%


==> Figures/Layout/Case2.tex <==
\begin{figure}[!tp]

    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim2_STV/WT_Sim2_STV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim2_STV/WT_Sim2_STV_tvsJ".pdf}}%

    \caption{Case 2. \TextFigureJa}%
    \label{fig:WT_Sim2_STV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%  

    \begin{minipage}{0.80\textwidth}%    

    \centering%      

        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim2_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.75".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/WT_Sim2_STV/WT_Sim2_STV_Newton".pdf}%   

    \end{minipage}%
    \subfloatcolorbar{0.0cm}{-1.275cm}{2.55cm}{"Figures/WT_Sim2_STV/WT_Sim2_STV_Colorbar".pdf}%
    \caption{Case 2. \TextRecosa}%
    \label{fig:WT_Sim2_STV_Recos}%
\end{figure}%


==> Figures/Layout/Case2_all.tex <==
\begin{figure}[!tp]%
\centering%  

    \begin{minipage}{0.80\textwidth}%    

    \centering%      

        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim2_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.5".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.75".pdf}%         

        

        \subfloatreco{\ttAlgd}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim2_STV/WT_Sim2_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/WT_Sim2_STV/WT_Sim2_STV_Newton".pdf}%   

    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/WT_Sim2_STV/WT_Sim2_STV_Colorbar".pdf}%
    \caption{Case 2. \TextRecosalla}%
    \label{fig:WT_Sim2_STV_Recosall}%
\end{figure}%



==> Figures/Layout/Case3.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim2_TV/WT_Sim2_TV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim2_TV/WT_Sim2_TV_tvsJ".pdf}}%

    \caption{Case 3. \TextFigureJb}

    \label{fig:WT_Sim2_TV_J}
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim2_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.75".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w1".pdf}%
        \subfloatreco{\ttAlgg}{"Figures/WT_Sim2_TV/WT_Sim2_TV_NLPDPS".pdf}%
    \end{minipage}%
    \subfloatcolorbar{0.0cm}{-1.275cm}{2.55cm}{"Figures/WT_Sim2_TV/WT_Sim2_TV_Colorbar".pdf}%
    \caption{Case 3. \TextRecosb}%
    \label{fig:WT_Sim2_TV_Recos}%
\end{figure}%


==> Figures/Layout/Case3_all.tex <==
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim2_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.5".pdf}%        
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.75".pdf}%  
        
        \subfloatreco{\ttAlgd}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim2_TV/WT_Sim2_TV_w1".pdf}%
        \subfloatreco{\ttAlgg}{"Figures/WT_Sim2_TV/WT_Sim2_TV_NLPDPS".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/WT_Sim2_TV/WT_Sim2_TV_Colorbar".pdf}%
    \caption{Case 4. \TextRecosallb}%
    \label{fig:WT_Sim2_TV_Recosall}%
\end{figure}%


==> Figures/Layout/Case4.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_tvsJ".pdf}}%

    \caption{Case 4. \TextFigureJa}%
    \label{fig:Skin_Meas1_STV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas1_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.75".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_Newton".pdf}%
    \end{minipage}%
    \subfloatcolorbar{0.0cm}{-1.2cm}{2.4cm}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_Colorbar".pdf}%
    \caption{Case 4. \TextRecosd}%

    \label{fig:Skin_Meas1_STV_Recos}%
\end{figure}%


==> Figures/Layout/Case4_all.tex <==
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas1_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.5".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.75".pdf}%     

        

        \subfloatreco{\ttAlgd}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_Newton".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/Skin_Meas1_STV/Skin_Meas1_STV_Colorbar".pdf}%
    \caption{Case 4. \TextRecosalld}%
    \label{fig:Skin_Meas1_STV_Recosall}%
\end{figure}%


==> Figures/Layout/Case5.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJb]{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_tvsJ".pdf}}%

    \caption{Case 5. \TextFigureJc}%
    \label{fig:Skin_Meas1_TV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \hspace{-1.5cm}\subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas1_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.75".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1.9cm}{-1.2cm}{2.4cm}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_Colorbar".pdf}%
    \caption{Case 5. \TextRecose}%
    \label{fig:Skin_Meas1_TV_Recos}%
\end{figure}%


==> Figures/Layout/Case5_all.tex <==
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoi{\ttTrue}{0.167\textwidth}{"Figures/Photos/Skin_Meas1_True".jpg}%
        \subfloatreco{\ttAlga}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.5".pdf}% 
        
        \subfloatreco{\ttAlgc}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.75".pdf}%
        \subfloatreco{\ttAlgd}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_w1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-2cm}{-2.75cm}{5.5cm}{"Figures/Skin_Meas1_TV/Skin_Meas1_TV_Colorbar".pdf}%
    \caption{Case 5. \TextRecosalle}%
    \label{fig:Skin_Meas1_TV_Recosall}%
\end{figure}%


==> Figures/Layout/Case6.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT3D_Sim1/WT3D_Sim1_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT3D_Sim1/WT3D_Sim1_tvsJ".pdf}}%

    \caption{Case 6. \TextFigureJc}%
    \label{fig:WT3D_Sim1_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \hspace{-1.25cm}\subfloatrecoii{\ttTrue}{0.4cm}{0.145\textwidth}{"Figures/WT3D_True/WT3D_True_view1".pdf}%
        \subfloatrecoii{\ttAlga}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.25_view1".pdf}%
        \subfloatrecoii{\ttAlgc}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.75_view1".pdf}%
        \subfloatrecoii{\ttAlge}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w1_view1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1.55cm}{-1.275cm}{2.5cm}{"Figures/WT3D_Sim1/WT3D_Sim1_Colorbar".pdf}%
    \caption{Case 6. \TextRecosg}%

    \label{fig:WT3D_Meas1_View1_Recos}%
\end{figure}%


==> Figures/Layout/Case6_all.tex <==
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatrecoii{\ttTrue}{0.4cm}{0.145\textwidth}{"Figures/WT3D_True/WT3D_True_view1".pdf}%
        \subfloatrecoii{\ttAlga}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.25_view1".pdf}%
        \subfloatrecoii{\ttAlgb}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.5_view1".pdf}%
        \\\subfloatrecoii{\ttAlgc}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.75_view1".pdf}%
        \subfloatrecoii{\ttAlgd}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w0.9_view1".pdf}%
        \subfloatrecoii{\ttAlge}{0.4cm}{0.145\textwidth}{"Figures/WT3D_Sim1/WT3D_Sim1_w1_view1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-2cm}{-2.75cm}{5.5cm}{"Figures/WT3D_Sim1/WT3D_Sim1_Colorbar".pdf}%
    \caption{Case 6. \TextRecosallg}%
    \label{fig:WT3D_Meas1_View1_Recosall}%
\end{figure}%


==> Figures/Layout/Case7.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim3_STV/WT_Sim3_STV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim3_STV/WT_Sim3_STV_tvsJ".pdf}}%

    \caption{Case 7. \TextFigureJa}%
    \label{fig:WT_Sim3_STV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim3_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim3_STV/WT_Sim3_STV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/WT_Sim3_STV/WT_Sim3_STV_w0.5".pdf}%
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim3_STV/WT_Sim3_STV_w0.75".pdf}%     

        

        \subfloatreco{\ttAlgd}{"Figures/WT_Sim3_STV/WT_Sim3_STV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim3_STV/WT_Sim3_STV_w1".pdf}%
        \subfloatreco{\ttAlgf}{"Figures/WT_Sim3_STV/WT_Sim3_STV_Newton".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/WT_Sim3_STV/WT_Sim3_STV_Colorbar".pdf}%
    \caption{Case 7. \TextRecosalla}%
    \label{fig:WT_Sim3_STV_Recos}%
\end{figure}%


==> Figures/Layout/Case8.tex <==
\begin{figure}[!tp]%
    \centering%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim3_TV/WT_Sim3_TV_kvsJ".pdf}}%
    \subfloat{\includegraphics[width=\figsizeJ]{"Figures/WT_Sim3_TV/WT_Sim3_TV_tvsJ".pdf}}%

    \caption{Case 8. \TextFigureJc}%
    \label{fig:WT_Sim3_TV_J}%
\end{figure}%
\begin{figure}[!tp]%
\centering%
    \begin{minipage}{0.80\textwidth}%
    \centering%
        \subfloatreco{\ttTrue}{"Figures/WT_True/Sim3_True".pdf}%
        \subfloatreco{\ttAlga}{"Figures/WT_Sim3_TV/WT_Sim3_TV_w0.25".pdf}%
        \subfloatreco{\ttAlgb}{"Figures/WT_Sim3_TV/WT_Sim3_TV_w0.5".pdf}%
        
        \subfloatreco{\ttAlgc}{"Figures/WT_Sim3_TV/WT_Sim3_TV_w0.75".pdf}%  
        \subfloatreco{\ttAlgd}{"Figures/WT_Sim3_TV/WT_Sim3_TV_w0.9".pdf}%
        \subfloatreco{\ttAlge}{"Figures/WT_Sim3_TV/WT_Sim3_TV_w1".pdf}%
    \end{minipage}%
    \subfloatcolorbar{-1cm}{-2.75cm}{5.5cm}{"Figures/WT_Sim3_TV/WT_Sim3_TV_Colorbar".pdf}%
    \caption{Case 8. \TextRecosallc}%
    \label{fig:WT_Sim3_TV_Recos}%
\end{figure}%


==> Tables/Parameters.tex <==
\begin{table}[!tp]
\hspace{0.5cm}
\caption{Parameters used in each test case. $\sigma^\text{ref}$ is the value of the homogeneous estimate computed from reference measurements.}\label{tab:Parameters}
    \resizebox{\columnwidth}{!}{
    \centering    
    \begin{tabular}{ l| c c c c c c c c c c  c}
        Case(s) & Setup & Data  & Regularisation & $L_A(i,i)$ &$\alpha$ & $l_\textbf{min}$ & $l_\textbf{max}$ & $\sigma_\textbf{min}$ & $\sigma_\textbf{max}$ & $V_\textbf{min}$ & $V_\textbf{max}$ \\
        \hline
        \hline    
        1           & 2D Water tank & Synthetic     & Smooth        & $5\cdot 10^4$ & -     & $10^{2} \sqrt{ 2 J(\sigma^1)}$                 & --                                & $10^{-4}$ & --                & $10^{-8}$ & $10^{12}$\\
        2      & 2D Water tank & Synthetic     & Smoothed TV   & $5\cdot 10^4$ & $10$  & $10^{2} \sqrt{ 2 J(\sigma^1)}$                 & $10^{2} \sqrt{ 2 J(\sigma^1)}$         & $10^{-4}$ & $10^{10}$         & $10^{-8}$ & $10^{12}$\\
        3      & 2D Water tank & Synthetic     & TV            & $5\cdot 10^4$ & $10$  & --                                        & --                                & -         & --                & $10^{-4}$ & $10^{12}$\\
        %3 \& 7      & 2D Water tank & Measured      & TV            & $5\cdot 10^4$ & $10$  & --                                        & --                                & -         & --                & $10^{-4}$ & $10^{12}$\\
        4      & Sensing skin  & Measured      & Smoothed TV   & $100$         & $1/4$ & $5 \sqrt{2J(\sigma^1)}$                   & $10^{-1} \sqrt{2J(\sigma^1)}$                & $10^{-4}$ & $\sigma^\textbf{ref}$  & $10^{-8}$ & $10^{12}$\\
        5    & Sensing skin  & Measured      & TV            & $100$         & $1/4$ & --                                        & --                                & -         & --                & $10^{-4}$ & $\sigma^\textbf{ref}$\\
        6          & 3D Water tank & Synthetic     & TV            & $5\cdot 10^4$ & $10$  & --                                        & --                                & -         & --                & $10^{-4}$ & $10^{12}$
\end{tabular}
}
\end{table}

==> Tables/Skin_Meas1_STV.tex <==
\begin{table}[!tp]
    \caption{Case 4. \textTabled}\label{table:SkinMeas1STV}
    \centering    
    \begin{tabular}{ l| c c  c  }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) \\
        \hline
        \hline    
        \ttAlgat&43&29478&1791.2 \\
        \ttAlgbt&37&29504&1538.9 \\
        \ttAlgct&23&29681&950.08 \\    
        \ttAlgdt&23&29858&954.99 \\
        \ttAlget&17&29679&676.2 \\        
        \ttAlgft&112&29949&1642.3
    \end{tabular}
\end{table}

==> Tables/Skin_Meas1_TV.tex <==
\begin{table}[!tp]
	\caption{Case 5. \textTablee}\label{table:SkinMeas1TV}
    \centering    
    \begin{tabular}{ l| c c  c  }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) \\
        \hline
        \hline
        \ttAlgat&44&37601&1256.8\\
        \ttAlgbt&26&37629&750.21 \\ 
        \ttAlgct&19&37801&540.46 \\
        \ttAlgdt&19&37812&531.91 \\
        \ttAlget&11&38015&299.03         
    \end{tabular}

\end{table}

==> Tables/Skin_Meas2_STV.tex <==
\begin{table}[!tp]
	\caption{Case 11. \textTabled}\label{table:SkinMeas2STV}
    \centering    
    \begin{tabular}{ l| c c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) \\
        \hline
        \hline
        \ttAlgat&65&23011&2747.8 \\
        \ttAlgbt&19&23262&775.53 \\ 
        \ttAlgct&11&23365&436.94 \\
        \ttAlgdt&29&23533&1206.2 \\
        \ttAlget&8&24544&311.8 \\    
        \ttAlgft&69&23072&1188.2
    \end{tabular}

\end{table}

==> Tables/Skin_Meas2_TV.tex <==
\begin{table}[!tp]
	\caption{Case 12. \textTablee}\label{table:SkinMeas2TV}	
    \centering    
    \begin{tabular}{ l| c c  c  }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) \\
        \hline
        \hline
        \ttAlgat&43&28761&1235.8\\
        \ttAlgbt&33&28984&950.35 \\
        \ttAlgct&16&29042&460.37 \\
        \ttAlgdt&14&29280&412.17 \\
        \ttAlget&14&30021&394.34    
    \end{tabular}
\end{table}

==> Tables/WT3D_Sim1.tex <==
\begin{table}[!tp]
    \caption{Case 6. \textTableb}\label{table:WT3DSim1}
    \centering    
    \begin{tabular}{ l| c c  c  c }
    Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
    \hline
    \hline
    \ttAlgat&47&300.5643&$1.6681\cdot 10^{4}$&2.8742\\
    \ttAlgbt&24&300.6393&$8.4881\cdot 10^{3}$&2.8737\\
    \ttAlgct&13&300.8226&$4.6491\cdot 10^{3}$&2.8768\\
    \ttAlgdt&12&301.1563&$4.3054\cdot 10^{3}$&2.8752 \\
    \ttAlget&9&300.6904&$3.2748\cdot 10^{3}$&2.8747
\end{tabular}
\end{table}

==> Tables/WT_Sim1.tex <==
\begin{table}[!tp]
    \centering    
    \caption{Case 1. \textTablea}    
    \begin{tabular}{ l| c c  c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
        \hline
        \hline        
        \ttAlgat&34&84.069&1197.4&2.1864\\
        \ttAlgbt&19&84.059&642.58&2.1895\\
        \ttAlgct&12&84.512&398.23&2.1975\\
        \ttAlgdt&8&$1.1179\cdot 10^8$&254.1&73.431\\
        \ttAlget&8&$4.5842\cdot 10^8$&255.97&103.68\\        
        \ttAlgft&14&86.7&2236.2&2.1969
    \end{tabular}
\label{table:WTSim1}
\end{table}

==> Tables/WT_Sim2_STV.tex <==
\begin{table}[!tbp]
    \centering    
    \caption{Case 2. \textTablea}\label{table:WTSim2STV}    
    \begin{tabular}{ l| c c  c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
        \hline
        \hline    
        \ttAlgat&31&135.35&1033.7&6.5056\\
        \ttAlgbt&15&135.61&487.21&6.5088\\    
        \ttAlgct&10&135.51&315.76&6.5164\\
        \ttAlgdt&10&135.63&319.6&6.5162\\
        \ttAlget&8&$5.386\cdot 10^8$&275.66&151.06\\        
        \ttAlgft&13&135.77&2622.4&7.1371
    \end{tabular}
\end{table}

==> Tables/WT_Sim2_TV.tex <==
\begin{table}[!tbp]
    \caption{Case 3. \textTableb}\label{table:WTSim2TV}
    \centering    
    \begin{tabular}{ l| c c  c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
        \hline
        \hline
        \ttAlgat&31&129.48&935.31&5.8401\\
        \ttAlgbt&16&129.97&473.62&5.8436 \\
        \ttAlgct&11&129.9&313.4&5.8466 \\ 
        \ttAlgdt&11&130.24&314.73&5.8533 \\
        \ttAlget&8&$7.1417\cdot 10^8$&225.87&334.68 \\
        \ttAlggt&24221&130.56&$9.9253\cdot 10^5$&5.9157        
    \end{tabular}
\end{table}

==> Tables/WT_Sim3_STV.tex <==
\begin{table}[!tp]
    \caption{Case 7. \textTablea}\label{table:WTSim3STV}
    \centering    
    \begin{tabular}{ l| c c  c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
        \hline
        \hline    
        \ttAlgat&34&73.942&1145.2&10.012\\    
        \ttAlgbt&16&74.238&526.82&10.035\\
        \ttAlgct&11&74.02&342.07&10.069\\
        \ttAlgdt&8&$4.5458\cdot 10^8$&235.21&166.67\\
        \ttAlget&8&$6.3257\cdot 10^8$&243.83&295.45\\        
        \ttAlgft&12&80.658&2387.1&11.161
\end{tabular}
\end{table}

==> Tables/WT_Sim3_TV.tex <==
\begin{table}[!tbp]
    \caption{Case 5. \textTablec}\label{table:WTSim3TV}
    \centering    
    \begin{tabular}{ l| c c  c  c }
        Algorithm  & Iterations $(K)$ & $J(\hz)$ & Time (s) & RE(\%) \\
        \hline
        \hline
        \ttAlgat&34&69.493&1025.7&8.6152\\
        \ttAlgbt&16&70.155&498.23&8.6516 \\
        \ttAlgct&12&69.57&367.28&8.6591 \\
        \ttAlgdt&8&5.2339$\cdot 10^8$&234.4&157.91 \\
        \ttAlget&8&6.6964$\cdot 10^8$&239.45&346.57
    \end{tabular}
\end{table}
